A Family of Independent Variable Eddington Factor Methods with Efficient Preconditioned Iterative Solvers

We present a family of discretizations for the Variable Eddington Factor (VEF) equations that have high-order accuracy on curved meshes and efficient preconditioned iterative solvers. The VEF discretizations are combined with a high-order Discontinuous Galerkin transport discretization to form an effective high-order, linear transport method. The VEF discretizations are derived by extending the unified analysis of Discontinuous Galerkin methods for elliptic problems to the VEF equations. This framework is used to define analogs of the interior penalty, second method of Bassi and Rebay, minimal dissipation local Discontinuous Galerkin, and continuous finite element methods. The analysis of subspace correction preconditioners, which use a continuous operator to iteratively precondition the discontinuous discretization, is extended to the case of the non-symmetric VEF system. Numerical results demonstrate that the VEF discretizations have arbitrary-order accuracy on curved meshes, preserve the thick diffusion limit, and are effective on a proxy problem from thermal radiative transfer in both outer transport iterations and inner preconditioned linear solver iterations. In addition, a parallel weak scaling study of the interior penalty VEF discretization demonstrates the scalability of the method out to 1152 processors.

==> figs/cp_zas2.tex <==
\begin{tabular}{ccccccc}
\toprule
 & $N_e$ & IP & BR2 & MDLDG & CG \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$p=1$}} & 112 & 10 & 10 & 14 & 10 \\
 & 448 & 11 & 11 & 16 & 12 \\
 & 1792 & 13 & 13 & 16 & 13 \\
 & 7168 & 14 & 14 & 18 & 14 \\
\addlinespace
\multirow{4}{*}{\rotatebox{90}{$p=2$}} & 112 & 13 & 13 & 16 & 13 \\
 & 448 & 15 & 15 & 18 & 15 \\
 & 1792 & 16 & 16 & 18 & 16 \\
 & 7168 & 17 & 17 & 19 & 17 \\
\addlinespace
\multirow{4}{*}{\rotatebox{90}{$p=3$}} & 112 & 15 & 15 & 17 & 15 \\
 & 448 & 16 & 16 & 18 & 16 \\
 & 1792 & 17 & 17 & 19 & 17 \\
 & 7168 & 18 & 18 & 19 & 18 \\
\bottomrule
\end{tabular}

==> figs/cp_zas2_1.tex <==
\begin{tabular}{cccccccccccccccccc}
\toprule
 &  & \multicolumn{3}{c}{IP}  &  & \multicolumn{3}{c}{BR2}  &  & \multicolumn{3}{c}{MDLDG}  &  & \multicolumn{3}{c}{CG} \\
\cmidrule{3-5}\cmidrule{7-9}\cmidrule{11-13}\cmidrule{15-17}
 & $N_e$ & Max & Min & Avg. & & Max & Min & Avg. & & Max & Min & Avg. & & Max & Min & Avg. \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$p=1$}} & 112 & 16 & 6 & 11.50 & & 16 & 6 & 11.20 & & 10 & 3 & 6.43 & & 7 & 3 & 4.90 \\
 & 448 & 17 & 7 & 12.00 & & 16 & 7 & 11.18 & & 11 & 3 & 6.94 & & 7 & 2 & 4.75 \\
 & 1792 & 18 & 4 & 11.23 & & 18 & 4 & 11.00 & & 11 & 4 & 7.38 & & 7 & 2 & 4.85 \\
 & 7168 & 18 & 6 & 11.50 & & 17 & 6 & 11.21 & & 12 & 3 & 6.94 & & 8 & 2 & 5.00 \\
\addlinespace
\multirow{4}{*}{\rotatebox{90}{$p=2$}} & 112 & 16 & 5 & 10.69 & & 16 & 5 & 10.85 & & 11 & 4 & 7.62 & & 9 & 3 & 6.23 \\
 & 448 & 17 & 5 & 11.20 & & 17 & 5 & 10.80 & & 12 & 4 & 7.94 & & 10 & 3 & 6.07 \\
 & 1792 & 17 & 4 & 11.12 & & 16 & 4 & 11.12 & & 14 & 4 & 9.11 & & 10 & 3 & 6.38 \\
 & 7168 & 17 & 5 & 11.18 & & 19 & 5 & 11.35 & & 14 & 4 & 9.32 & & 11 & 3 & 6.41 \\
\addlinespace
\multirow{4}{*}{\rotatebox{90}{$p=3$}} & 112 & 19 & 5 & 12.47 & & 18 & 6 & 12.20 & & 22 & 5 & 12.29 & & 11 & 3 & 7.53 \\
 & 448 & 22 & 7 & 14.00 & & 18 & 6 & 13.19 & & 17 & 6 & 11.61 & & 12 & 5 & 8.56 \\
 & 1792 & 22 & 6 & 14.06 & & 22 & 6 & 14.35 & & 18 & 6 & 12.58 & & 13 & 4 & 8.71 \\
 & 7168 & 22 & 7 & 14.39 & & 20 & 7 & 14.17 & & 20 & 7 & 12.95 & & 13 & 4 & 9.11 \\
\bottomrule
\end{tabular}

==> figs/cp_zas2_2.tex <==
\begin{tabular}{cccccccccccc}
\toprule
 &  & \multicolumn{4}{c}{Avg.~Assembly Time (ms)}  &  & \multicolumn{4}{c}{Avg.~VEF Solve Time (ms)} \\
\cmidrule{3-6}\cmidrule{8-11}
 & $N_e$ & IP & BR2 & MDLDG & CG & & IP & BR2 & MDLDG & CG \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$p=1$}} & 112 & 11.75 & 13.40 & 10.66 & 11.88 & & 1.40 & 1.40 & 1.90 & 0.89 \\
 & 448 & 45.16 & 52.42 & 40.45 & 45.35 & & 5.03 & 4.92 & 7.87 & 3.22 \\
 & 1792 & 179.70 & 201.69 & 159.04 & 180.08 & & 18.97 & 18.47 & 31.59 & 12.29 \\
 & 7168 & 702.14 & 813.73 & 630.44 & 722.46 & & 75.65 & 74.72 & 122.41 & 48.72 \\
\addlinespace
\multirow{4}{*}{\rotatebox{90}{$p=2$}} & 112 & 23.20 & 28.37 & 22.36 & 23.24 & & 3.49 & 3.49 & 4.76 & 1.99 \\
 & 448 & 88.47 & 110.46 & 85.85 & 89.50 & & 13.32 & 13.11 & 18.65 & 7.44 \\
 & 1792 & 355.21 & 444.23 & 343.34 & 363.72 & & 53.87 & 53.56 & 80.18 & 29.46 \\
 & 7168 & 1414.84 & 1796.56 & 1390.85 & 1449.62 & & 213.06 & 217.13 & 323.86 & 117.62 \\
\addlinespace
\multirow{4}{*}{\rotatebox{90}{$p=3$}} & 112 & 43.98 & 62.49 & 46.48 & 43.49 & & 9.45 & 9.41 & 15.41 & 5.04 \\
 & 448 & 172.69 & 251.23 & 187.84 & 175.26 & & 41.42 & 39.23 & 61.63 & 21.56 \\
 & 1792 & 685.62 & 1018.82 & 756.87 & 712.72 & & 161.52 & 164.56 & 257.24 & 87.83 \\
 & 7168 & 2920.94 & 4233.22 & 3110.92 & 2922.78 & & 735.27 & 714.31 & 1109.79 & 359.74 \\
\bottomrule
\end{tabular}

==> figs/cp_zas2_3.tex <==
\begin{tabular}{ccccccccccccccccc}
\toprule
 &  & \multicolumn{4}{c}{Total Solve Time (s)}  &  & \multicolumn{4}{c}{Sweep Time (s)}  &  & \multicolumn{4}{c}{VEF Time (s)} \\
\cmidrule{3-6}\cmidrule{8-11}\cmidrule{13-16}
 & $N_e$ & IP & BR2 & MDLDG & CG & & IP & BR2 & MDLDG & CG & & IP & BR2 & MDLDG & CG \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$p=1$}} & 112 & 1.79 & 1.81 & 2.48 & 1.79 & & 1.66 & 1.66 & 2.30 & 1.66 & & 0.13 & 0.15 & 0.18 & 0.13 \\
 & 448 & 6.70 & 6.82 & 9.54 & 7.27 & & 6.13 & 6.17 & 8.75 & 6.67 & & 0.56 & 0.64 & 0.78 & 0.59 \\
 & 1792 & 30.23 & 30.23 & 36.70 & 29.88 & & 27.58 & 27.30 & 33.59 & 27.32 & & 2.64 & 2.92 & 3.11 & 2.55 \\
 & 7168 & 127.70 & 128.94 & 163.07 & 126.04 & & 116.41 & 116.05 & 148.93 & 114.92 & & 11.23 & 12.85 & 13.96 & 11.08 \\
\addlinespace
\multirow{4}{*}{\rotatebox{90}{$p=2$}} & 112 & 3.87 & 3.92 & 4.74 & 3.82 & & 3.51 & 3.49 & 4.29 & 3.48 & & 0.36 & 0.42 & 0.44 & 0.33 \\
 & 448 & 16.05 & 16.30 & 19.36 & 15.99 & & 14.45 & 14.38 & 17.42 & 14.50 & & 1.57 & 1.90 & 1.92 & 1.48 \\
 & 1792 & 67.49 & 68.88 & 75.92 & 66.87 & & 60.64 & 60.61 & 68.08 & 60.38 & & 6.78 & 8.19 & 7.82 & 6.47 \\
 & 7168 & 284.28 & 289.36 & 317.42 & 283.65 & & 255.21 & 253.67 & 283.78 & 255.82 & & 28.84 & 35.49 & 33.54 & 27.54 \\
\addlinespace
\multirow{4}{*}{\rotatebox{90}{$p=3$}} & 112 & 8.93 & 9.18 & 10.20 & 8.84 & & 8.10 & 8.07 & 9.13 & 8.10 & & 0.82 & 1.10 & 1.07 & 0.74 \\
 & 448 & 37.06 & 37.88 & 41.87 & 36.51 & & 33.49 & 33.11 & 37.30 & 33.28 & & 3.53 & 4.76 & 4.56 & 3.21 \\
 & 1792 & 154.65 & 161.33 & 175.43 & 154.59 & & 139.61 & 140.46 & 155.67 & 140.26 & & 14.98 & 20.83 & 19.71 & 13.99 \\
 & 7168 & 676.70 & 706.40 & 721.94 & 673.00 & & 607.85 & 614.35 & 638.54 & 612.08 & & 68.62 & 91.86 & 82.04 & 60.75 \\
\bottomrule
\end{tabular}

==> figs/cp_zas2_4.tex <==
\begin{tabular}{ccccccc}
\toprule
 & $N_e$ & IP & BR2 & MDLDG & CG \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$p=1$}} & 112 & 15.166 & 15.606 & 11.091 & 16.588 \\
 & 448 & 5.417 & 5.781 & 4.379 & 7.269 \\
 & 1792 & 2.353 & 2.346 & 2.101 & 2.622 \\
 & 7168 & 1.248 & 1.242 & 1.275 & 1.257 \\
\addlinespace
\multirow{4}{*}{\rotatebox{90}{$p=2$}} & 112 & 15.533 & 17.473 & 13.336 & 17.756 \\
 & 448 & 6.769 & 7.151 & 5.776 & 7.673 \\
 & 1792 & 3.185 & 3.184 & 2.964 & 3.272 \\
 & 7168 & 1.979 & 1.977 & 1.954 & 1.981 \\
\addlinespace
\multirow{4}{*}{\rotatebox{90}{$p=3$}} & 112 & 20.809 & 21.404 & 15.941 & 21.770 \\
 & 448 & 8.475 & 8.693 & 7.218 & 8.932 \\
 & 1792 & 4.722 & 4.723 & 4.488 & 4.733 \\
 & 7168 & 2.765 & 2.768 & 2.703 & 2.764 \\
\bottomrule
\end{tabular}

==> figs/dsacomp.tex <==
\begin{tabular}{cccc}
\toprule
$h_\mathrm{min}$ & $h_\mathrm{max}$ & $\| \varphi_\mathrm{VEF} - \varphi_\mathrm{SN}\|$ \\
\midrule
\num{3.855e-04} & \num{1.963e-02} & \num{1.230e-06} \\
\num{2.467e-04} & \num{1.571e-02} & \num{6.605e-07} \\
\num{1.713e-04} & \num{1.309e-02} & \num{3.949e-07} \\
\num{1.259e-04} & \num{1.122e-02} & \num{2.547e-07} \\
\num{9.638e-05} & \num{9.817e-03} & \num{1.737e-07} \\
\bottomrule
\end{tabular}

==> figs/dsacompcp.tex <==
\begin{tabular}{cccc}
\toprule
$h_\mathrm{min}$ & $h_\mathrm{max}$ & $\| \varphi_\mathrm{VEF} - \varphi_\mathrm{SN}\|$ \\
\midrule
\num{8.540e-03} & \num{1.118e-01} & \num{6.292e-02} \\
\num{4.269e-03} & \num{5.590e-02} & \num{3.688e-02} \\
\num{2.113e-03} & \num{2.795e-02} & \num{2.045e-02} \\
\num{1.067e-03} & \num{1.398e-02} & \num{1.045e-02} \\
\bottomrule
\end{tabular}

==> figs/strong_1.tex <==
\begin{tabular}{cccccc}
\toprule
Processors & Total & Sweep & VEF Solve & VEF Assembly \\
\midrule
1 & 3355.785 & 3012.825 & 44.555 & 277.206 \\
2 & 1994.637 & 1787.598 & 29.002 & 165.633 \\
4 & 1266.370 & 1133.720 & 20.516 & 103.105 \\
8 & 786.596 & 705.586 & 13.679 & 62.889 \\
16 & 486.479 & 436.586 & 9.162 & 38.100 \\
32 & 345.736 & 308.878 & 8.874 & 26.220 \\
\bottomrule
\end{tabular}

==> figs/tgmms2.tex <==
\num{6.259e-02} &  & \num{7.988e-04} & \num{7.973e-04} & \num{7.417e-04} & \num{8.076e-04} &  & \num{2.610e-05} \\
\num{4.173e-02} &  & \num{2.457e-04} & \num{2.441e-04} & \num{2.337e-04} & \num{2.477e-04} &  & \num{5.421e-06} \\
\num{3.130e-02} &  & \num{1.048e-04} & \num{1.038e-04} & \num{9.990e-05} & \num{1.054e-04} &  & \num{2.143e-06} \\
\num{2.504e-02} &  & \num{5.387e-05} & \num{5.327e-05} & \num{5.152e-05} & \num{5.415e-05} &  & \num{1.021e-06} 

==> figs/tgmms2_1.tex <==
Order &  & 2.943 & 2.953 & 2.911 & 2.949 \\
Constant &  & 2.793 & 2.868 & 2.384 & 2.874 

==> figs/weak_cp1.tex <==
\begin{tabular}{cccccc}
\toprule
Processors & DOF & Diffusion & AMG & AMG-S \\
\midrule
36 & \num{326592} & 15 & 20 & 20 \\
72 & \num{630000} & 14 & 19 & 20 \\
144 & \num{1306368} & 13 & 20 & 18 \\
288 & \num{2570652} & 15 & 22 & 18 \\
576 & \num{5225472} & 15 & 22 & 20 \\
864 & \num{7805952} & 15 & 22 & 21 \\
1152 & \num{10384668} & 16 & 22 & 21 \\
\bottomrule
\end{tabular}

==> figs/weak_cp2.tex <==
\begin{tabular}{cccccc}
\toprule
Processors & DOF & Diffusion & AMG & AMG-S \\
\midrule
36 & \num{326592} & 15 & 20 & 20 \\
72 & \num{630000} & 14 & 19 & 20 \\
144 & \num{1306368} & 13 & 20 & 18 \\
288 & \num{2570652} & 15 & 22 & 18 \\
576 & \num{5225472} & 15 & 22 & 20 \\
864 & \num{7805952} & 15 & 22 & 21 \\
1152 & \num{10384668} & 16 & 22 & 21 \\
\bottomrule
\end{tabular}

==> figs/weak_cp3.tex <==
\begin{tabular}{cccccc}
\toprule
Processors & DOF & Diffusion & AMG & AMG-S \\
\midrule
36 & \num{326592} & 15 & 20 & 20 \\
72 & \num{630000} & 14 & 19 & 20 \\
144 & \num{1306368} & 13 & 20 & 18 \\
288 & \num{2570652} & 15 & 22 & 18 \\
576 & \num{5225472} & 15 & 22 & 20 \\
864 & \num{7805952} & 15 & 22 & 21 \\
1152 & \num{10384668} & 16 & 22 & 21 \\
\bottomrule
\end{tabular}

==> figs/weak_mock_t1.tex <==
\begin{tabular}{ccccccc}
\toprule
Processors & DOF & AMG & Direct & AMG-S & AMG-S3 \\
\midrule
36 & \num{326592} & -- & 22 & 25 & 20 \\
72 & \num{630000} & -- & 24 & 27 & 21 \\
144 & \num{1306368} & -- & 20 & 25 & 22 \\
288 & \num{2570652} & -- & 22 & 25 & 25 \\
576 & \num{5225472} & -- & 22 & 28 & 23 \\
864 & \num{7805952} & -- & 22 & 26 & 23 \\
1152 & \num{10384668} & -- & 21 & 29 & 27 \\
\bottomrule
\end{tabular}

==> figs/weak_mock_t2.tex <==
\begin{tabular}{ccccccc}
\toprule
Processors & DOF & AMG & Direct & AMG-S & AMG-S3 \\
\midrule
36 & \num{326592} & -- & 22 & 25 & 20 \\
72 & \num{630000} & -- & 24 & 27 & 21 \\
144 & \num{1306368} & -- & 20 & 25 & 22 \\
288 & \num{2570652} & -- & 22 & 25 & 25 \\
576 & \num{5225472} & -- & 22 & 28 & 23 \\
864 & \num{7805952} & -- & 22 & 26 & 23 \\
1152 & \num{10384668} & -- & 21 & 29 & 27 \\
\bottomrule
\end{tabular}

==> figs/weak_mock_t3.tex <==
\begin{tabular}{ccccccc}
\toprule
Processors & DOF & AMG & Direct & AMG-S & AMG-S3 \\
\midrule
36 & \num{326592} & -- & 22 & 25 & 20 \\
72 & \num{630000} & -- & 24 & 27 & 21 \\
144 & \num{1306368} & -- & 20 & 25 & 22 \\
288 & \num{2570652} & -- & 22 & 25 & 25 \\
576 & \num{5225472} & -- & 22 & 28 & 23 \\
864 & \num{7805952} & -- & 22 & 26 & 23 \\
1152 & \num{10384668} & -- & 21 & 29 & 27 \\
\bottomrule
\end{tabular}
